Active Bayesian Multi-class Mapping from Range and Semantic Segmentation Observation

Many robot applications call for autonomous exploration and mapping of unknown and unstructured environments. Information-based exploration techniques, such as Cauchy-Schwarz quadratic mutual information (CSQMI) and fast Shannon mutual information (FSMI), have successfully achieved active binary occupancy mapping with range measurements. However, as we envision robots performing complex tasks specified with semantically meaningful objects, it is necessary to capture semantic categories in the measurements, map representation, and exploration objective. This work develops a Bayesian multi-class mapping algorithm utilizing range-category measurements. We derive a closed-form efficiently computable lower bound for the Shannon mutual information between the multi-class map and the measurements. The bound allows rapid evaluation of many potential robot trajectories for autonomous exploration and mapping. We compare our method against frontier-based and FSMI exploration and apply it in a 3-D photo-realistic simulation environment.

==> tex/old/Mapping.tex <==
\section{Bayesian Multi-class Mapping}
\label{sec:bayes_multi_class_mapping}

The previous section defined likelihood of a sensor observation $z_t$ conditioned on the environment map $\bfm$. Here, we focus on the inverse problem, i.e., computing the posterior PDF $p_t(\bfm)$ of the map conditioned on an observation $z_t$.

% too lengthy propositions

\begin{proposition}
Bayesian multi-class mapping can be formulated as a recursive additive model. Let $\bfh_{t,i} = [0, h_{t,i,1}, \ldots, h_{t,i,K}]^T$ be the vector of multi-class log ratios. For each class $k \in \calK$ we have:
% j and i
\begin{equation}
\begin{aligned}
    h^{b}_{t,i,k} &= l_{i,k}(z_{t,b}) + h^{b-1}_{t,j,k} - l^0_k, &b = 1, \ldots, B \\
    h_{t,j,k} &= h^{B}_{t,j,k}, &h_{t-1,j,k} = h^{0}_{t,j,k}
\end{aligned}
\label{eq:semantic_logodds_mapping}
\end{equation}
%
where $h_{t,j,k}$ and $h^{b}_{t,j,k}$ are defined as:
%
\begin{equation}
\begin{aligned}
    h_{t,i,k} &= \log{\frac{p_t(m_i=k)}{p_t(m_i=0)}} \\ 
    h^{b}_{t,i,k} &= \log{\frac{p(m_i=k \mid z_{t,1:b}, \bfz_{1:t-1})}{p(m_i=0 \mid z_{t,1:b}, \bfz_{1:t-1})}}.
\end{aligned}
\end{equation}
%
\end{proposition}
%

Correctness of the proposition can be explained as follows. From the graphical model of Fig.~\ref{} we have:
%
\begin{equation}
    p_t(\bfm) = p(\bfm \mid \bfz_{1:t}) = \prod_{i=1}^N p(m_i \mid \bfz_{1:t}).
\end{equation}
%
Using the Bayes rule, this can be further decomposed to:
%
\begin{equation}
    p_t(\bfm) = \frac{p(z_t)}{p(z_t \mid \bfz_{1:t-1})} \prod_{i=1}^N \frac{p(m_i \mid z_t) p_{t-1}(m_i)}{p_0(m_i)}.
\end{equation}
%
In order to eliminate the unknown term $p(z_t \mid \bfz_{1:t-1})$, we consider the odds ratio of map probabilities:
%
\begin{equation}
\begin{split}
    &\prod_{i=1}^N \frac{p_t(m_i = k)}{p_t(m_i = 0)} = \\ &\prod_{i=1}^N \frac{p(m_i = k \mid z_t) p_{t-1}(m_i = k) p_0(m_i = 0)}{p(m_i = 0 \mid z_t) p_{t-1}(m_i = 0) p_0(m_i = k)}.
\end{split}
\end{equation}
%
Since each term in both the left and right products only depends on one map cell $m_i$, a similar equation holds for every single cell:
%
\begin{equation}
    \frac{p_t(m_i = k)}{p_t(m_i = 0)} = \frac{p(m_i = k \mid z_t) p_{t-1}(m_i = k) p_0(m_i = 0)}{p(m_i = 0 \mid z_t) p_{t-1}(m_i = 0) p_0(m_i = k)}.
\label{eq:semantic_mapping}
\end{equation}
%
Moreover, since our observation model is defined over a single beam, we describe the update rule for each beam $z_{t,b}$:
%
\begin{equation}
\begin{split}
    &\frac{p(m_i = k \mid z_{t,1:b}, \bfz_{1:t-1})}{p(m_i = 0 \mid z_{t,1:b}, \bfz_{1:t-1})} = \\ 
    &\frac{p(m_i = k \mid z_{t,b}) p(m_i = k \mid z_{t,1:b-1}, \bfz_{1:t-1}) p_0(m_i = 0)}{p(m_i = 0 \mid z_{t,b}) p(m_i = 0 \mid z_{t,1:b-1}, \bfz_{1:t-1}) p_0(m_i = k)}.
\end{split}
\end{equation}
%
Re-writing the above in logarithmic form results in a multi-class generalization of log-odds mapping as in Eq.~\eqref{eq:semantic_logodds_mapping}. Similar to the log ratio of the inverse observation model, class probabilities for each cell $m_i$ can be recovered by a softmax function as $p_t(m_i = k) = \sigma^k(h_{t,i,k})$.

By knowing how an observation $z_t$ could affect the map probability $p_t(\bfm)$, we now switch our focus to the computation of the mutual information between a sequence of observations $\bfz_{t+1:t+T}$ and the map $\bfm$.

==> tex/old/MutualInformationOctoMap.tex <==
\section{Information Computation for Semantic OctoMap Representation}
\label{sec:info_comp_octomap}

% high-level structure: semantic octomapping (map update + data structure + pruning strategy (not sure about the amount of details to be provided)) -> info computation using RLE -> complexity comparison with the full grid case

Full grid representation of 3D environments demands for expensive processing power and large memory requirements. However, the occupied space in realistic situations is usually distributed sparsely across the environment; while the free space comprises a large and continuous portion of the scene. The OctoMap \cite{octomap} technique exploits this property in order to provide an efficient variable-sized grid representation of a 3D environment. The OctoMap method combines many small cells associated with the free space into one large cell using an octree data structure; leading to significant gains in terms of memory usage and computational cost. In the following, we first provide a semantic version of the OctoMap technique. Next, we propose an efficient semantic mutual information formula which benefits from the structure of an OctoMap representation.

\subsection{Semantic Octomap}

An octree is a hierarchical data structure containing nodes that represent a section of the physical environment. Each node has either 0 or 8 children, where the latter corresponds to the 8 octants of the Euclidean 3-D coordinate system. Therefore, children of a node form a homogeneous partition of the space that the parent node corresponds to. The most basic type of an octree node stores occupancy probability of the region it represents. Based on our application requirements, we append RGB color and multi-class log ratios to the information carried by a node. This allows for a colored semantic representation of a 3-D environment where cell colors can switch between class label and actual object color.

In order to register a new observation to the OctoMap, we follow the standard ray-casting procedure over an octree \cite{octomap} to find the observed leaf nodes. Then, for each observed leaf node, the multi-class log ratios are updated using \eqref{eq:semantic_logodds_mapping}. For ray end point, which indicates an occupied cell, we also update the RGB color by averaging the observed color with the current stored color of the corresponding node. Inspired by \cite{semantic_octomap}, the multi-class log-odds vector for each node only stores the probabilities for the three most likely classes; while the probability of the rest of the object classes lump into a single \textit{others} class. This relives the semantic OctoMap implementation from dependence on the number of classes that the object classifier can detect. Moreover, it significantly helps to improve the performance of the mapping algorithm in cases where there is a large variety of object classes. Alg.~\ref{alg:fuse_obs} details the probabilistic observation fusion procedure for our semantic OctoMap.

It is necessary to define information propagation from children nodes towards parent (inner) nodes, so that a coarser representation of the OctoMap can be computed. This is useful for navigation where efficient collision checking is prioritized over detailed environment representation. Depending on the application, different information fusion strategies can be implemented. For example, a conservative strategy would assign multi-class log-odds of the child node with the most occupancy probability to the parent node. In this work, we simply assign the average log-odds vector of children nodes to their parent node as shown in Alg.~\ref{alg:semantic_fusion}.

As mentioned earlier, the main benefit of the OctoMap representation is the possibility of combining similar grid cells (leaf nodes) into a large cell (inner node). This is called \textit{pruning} the OctoMap. Every time after an observation is integrated to the map, we check for each node if \begin{inparaenum}[1)] \item the node has 8 children, \item its children don't have any children of their own, and \item its children all have equal multi-class log ratios. \end{inparaenum} In order to make pruning more likely to happen, we maintain thresholds for maximum and minimum multi-class log-odds values, as suggested by the original paper \cite{octomap}. For mapping using range sensors, this helps to compress a majority of the free cells into a few large cells; while occupied cells usually do not undergo pruning since only the surface of objects will be observed by the sensor, and their inside remains as \textit{unexplored} region.

\begin{algorithm}[t]
\caption{Semantic OctoMap Update}\label{alg:fuse_obs}
\begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE $\bfh_{t,i}$, $z_{t,b}$, $\alpha$
 \ENSURE $\bfh_{t+1,i}$
 \IF{$z_{t,b}$ indicates free}
 \STATE $\bfh_{t+1,i} = \bfh_{t,i} + \bfl^-$ // Assuming $\bfl^0 = \boldsymbol{0}$
 \ELSIF{$z_{t,b}$ indicates class $y_{t,b}$}
  \STATE // Check if class $y_{t,b}$ is among the 3 most likely classes in $\bfh_{t,i}$
 \IF{$y_{t,b} \in h_{t,i,1:3}$}
 \STATE $\bfh_{t+1,i} = \bfh_{t,i} + \bfl^+(y_{t,b})$
 \ELSE
 \STATE $h_{aux} = h_{t,i,4} + \log{\alpha}$ // Derive $h_{aux}$ as a portion $\alpha$ of \textit{others} class
 \STATE $h_{t,i,4} \mathrel{+}= \phi^+_{others} + \log{(1-\alpha)}$
 \STATE $\Tilde{\bfh} = concat(h_{t,i,1:3}, h_{aux})$
 \STATE $\Tilde{\bfh} \mathrel{+}= \bfl^+(y_{t,b})$
 \STATE $\Tilde{\bfh}^s = sort(\Tilde{\bfh})$ // Descending sort
 \STATE $h_{t+1,i,1:3} = \Tilde{h}^s_{1:3}$ // Pick 3 most likely classes
 \STATE $h_{t+1,i,4} = \log{\Big(\exp{(\Tilde{h}^s_{4})} + \exp{(h_{t,i,4})}\Big)}$ // Combine the least likely class with \textit{others} class
 \ENDIF
 \ENDIF
 \STATE $maxMinThresh(\bfh_{t+1,i})$ // Apply thresholds for maximum and minimum log-odds values
 \RETURN $\bfh_{t+1,i}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Semantic Fusion of Two Child Nodes}\label{alg:semantic_fusion}
\begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE $\bfh_i$, $\bfh_j$
 \ENSURE $\bfh_f$
 \FOR{$q \in \{i, j\}$}
 \STATE $\Bar{q} = \{i, j\} \setminus q$
 \STATE $n_q = 0$ // The number of classes in $h_{\Bar{q},1:3}$ which do not belong to $h_{q,1:3}$
 \FOR{$y \in h_{\Bar{q},1:3}$ and $y \notin h_{q,1:3}$}
 \STATE $n_q \mathrel{+}= 1$
 \ENDFOR
 \STATE $others_q = h_{q,4} - \log(1 + n_q)$ // Slice $h_{q,4}$ into smaller probabilities in order to fill $v_q$
 \STATE $v_q = h_{q,1:3}$
 \FOR{$n = 1:n_q$}
 \STATE $v_q.append(others_q)$
 \ENDFOR
 \ENDFOR
 \STATE $expOthers_f = \exp{(\frac{others_i + others_j}{2})}$
 \STATE $v_f = \frac{v_i + v_j}{2}$
 \STATE $sort(v_f)$ // Descending sort
 \STATE $h_{f,1:3} = v_{f,1:3}$ // Pick 3 most likely classes
 \FOR{$n > 3$ and $n \leq v_f.size$}
 \STATE $expOthers_f \mathrel{+}= \exp{(v_{f,n})}$ // Combine the remaining classes into \textit{others} class
 \ENDFOR
 \STATE $h_{f,4} = \log{(expOthers_f)}$
 \STATE $maxMinThresh(\bfh_f)$
 \RETURN $\bfh_f$
\end{algorithmic}
\end{algorithm}

\subsection{Information Computation}

A ray cast through an octree representation may visit several large (pruned) nodes where the class probabilities are homogeneous within each node. We exploit this property of an OctoMap in order to simplify the semantic information computation by redefining the mutual information between the OctoMap and a single ray as a summation over unique class probabilities, instead of individual map cells. As we will show in this section, this simplification provides a significant gain in terms of performance with minimal loss of accuracy. The following formulation can be considered as a multi-class generalization of the run-length encoding (RLE) technique introduced in \cite{fsmi}, using the semantic sensor model of Eq.~\eqref{eq:forward_obs_model_semantic_decomp} and the semantic OctoMap defined earlier in this section.

Assume that the map cells along a single beam have piece-wise constant class probabilities such that the set $\{m_i \mid i \in \calR(r_{max})\}$ can be partitioned into $Q$ groups of consecutive cells indexed by $\calR^q(r_{max})$ ($q = 1, \ldots, Q$) where:
%
\begin{equation}
\begin{split}
    p_t(m_i = k) = p_t(m_j = k), \\ i, j \in \calR^q(r_{max}), \;\;\; \forall k \in \calK.
\end{split}
\end{equation}
%
Fig~\ref{} shows an example for an environment with two object classes, i.e. $K = 2$.

This situation often happens within OctoMap representations; which delivers substantial gains in efficiency for mutual information computation since the contribution of each group $\{m_i \mid i \in \calR^q(r_{max})\}$ in the innermost summation of Eq.~\eqref{eq:mut_inf_semantic} can be obtained in closed form. Consider a single beam $z$, passing through cells $m_i$, $i \in \calR(r_{max})$. As shown in Sec.~\ref{sec:info_comp}, the mutual information between the map $\bfm$ and the beam $z$ can be computed as Eq.~\eqref{eq:mut_inf_single_ray}. Assuming piece-wise constant class probabilities, we have:
%
\begin{equation}
\begin{split}
    \sum_{n=1}^{N} p(n,k) C(n,k) &= \sum_{q=1}^Q \sum_{n= \omega_{1:q-1} + 1}^{\omega_{1:q}} p(n,k) C(n,k) \\
    &= \sum_{q=1}^Q IG(q,k)
\end{split}
\label{eq:piece_wise_const_info}
\end{equation}
%
where $\omega_q = | \calR^q(r_{max}) |$ and $\omega_{1:q} = \sum_{j=1}^q \omega_j$. For each $\omega_{1:q-1} < n \leq \omega_{1:q}$, we can simplify the terms $p(n,k)$ and $C(n,k)$ as follows:
%
\begin{equation}
    p(n,k) = \pi_t(q,k) \pi_t^{(n-1-\omega_{1:q-1})}(q,0) \prod_{j=1}^{q-1} \pi_t^{\omega_j}(j,0),
\end{equation}
\begin{equation}
\begin{split}
    C(n,k) = &f(\bfl^+(k), \bfchi_{t,q}) + \\ (n-1&-\omega_{1:q-1}) f(\bfl^-, \bfchi_{t,q}) + \sum_{j=1}^{q-1} \omega_j f(\bfl^-, \bfchi_{t,j}),
\end{split}
\end{equation}
%
where:
%
\begin{equation}
    \begin{cases} \pi_t(q,k) = p_t(m_i = k) \\ \bfchi_{t,q} = \bfh_{t,i} \end{cases} \;\; \forall i \in \calR^q(r_{max}).
\end{equation}
%
The simplification allows to find a closed form expression for the inner summation of Eq.~\eqref{eq:piece_wise_const_info}, namely the information gain $IG(q,k)$ as below:
%
\begin{equation}
\begin{split}
    IG(q,k) = \sum_{n= \omega_{1:q-1} + 1}^{\omega_{1:q}} &p(n,k) C(n,k) = \\ a_q(k) \big[&b_q(k) \sum_{j = 0}^{\omega_q - 1} \pi_t^{j}(q,0) + \\ &f(\bfl^-, \bfchi_{t,q}) \sum_{j = 0}^{\omega_q - 1} j \pi_t^j(q,0) \big],
\end{split}
\label{eq:within_section_sum}
\end{equation}
%
where $a_q(k)$ and $b_q(k)$ represent the following:
%
\begin{equation}
\begin{split}
    &a_q(k) = \pi_t(q,k) \prod_{j=1}^{q-1} \pi_t^{\omega_j}(j,0) \\
    &b_q(k) = f(\bfl^+(k), \bfchi_{t,q}) + \sum_{j=1}^{q-1} \omega_j f(\bfl^-, \bfchi_{t,j}).
\end{split}
\end{equation}
%
The summations in Eq.~\eqref{eq:within_section_sum} can be explicitly computed, leading to the following closed form expression:
%
\begin{equation}
\begin{split}
    &IG(q,k) = a_q(k) \big[b_q(k) \frac{1 - \pi_t^{\omega_q}(q,0)}{1 - \pi_t(q,0)} + \\ &f(\bfl^-, \bfchi_{t,q}) \frac{(\omega_q - 1) \pi_t^{\omega_q + 1}(q,0) - \omega_q \pi_t^{\omega_q}(q,0) + \pi_t(q,0)}{(1 - \pi_t(q,0))^2} \big] \\
\end{split}
\end{equation}
%
Therefore, the Shannon mutual information between a semantic OctoMap $\bfm$ and a sequence of future observations $\bfz_{t+1:t+T}$ can be computed as follows:
%
\begin{equation}
    I[\bfm; \bfz_{t+1:t+T} \mid \bfz_{1:t}] = \sum_{\tau=1}^{T} \sum_{b=1}^{B} \sum_{k=1}^K \sum_{q=1}^{Q_{\tau,b}} IG_{\tau,b}(q,k).
\label{eq:mut_inf_semantic_octomap}
\end{equation}
%

Going back to Eq.~\eqref{eq:mut_inf_semantic}, since the terms $p_{\tau,b}(n,k)$ and $C_{\tau,b}(n,k)$ can be computed recursively, the innermost summation can be calculated in $O(N_{\tau,b})$. This results in a complexity of $O(T B K N_{\tau,b})$ for the total information computation over a regular grid representation. Similarly, the terms $a_q(k)$ and $b_q(k)$ can be obtained recursively; which leads to a complexity of $O(T B K Q_{\tau,b})$ for the total information computation over an OctoMap representation. As we will discuss in section~\ref{sec:experiments}, the compactness of an OctoMap representation leads to arbitrary gain in performance reciprocal to the physical dimensions of leaf nodes. In other words, the computational complexity of a regular grid grows linearly with map resolution; while the complexity of information computation over an OctoMap remains almost independent of map resolution.

==> tex/old/SensorModel.tex <==
\section{Semantic Range Sensor Model}
\label{sec:semantic_range_sensor_model}

This section defines an inverse observation model for a range-category measurement $\bfz = (r,y)$ obtained from robot posisition $\bfp$ in the direction of a single sensor ray $\bfR \bfeta$. This model will be used in Sec.~\ref{sec:bayes_multi_class_mapping} to derive the Bayesian update in \eqref{eq:bayes_rule} for the semantic map PDF.

Let $\calR(\bfz ; \bfX, \bfeta) \subseteq \calI$ be a set of map indices corresponding to the map cells $m_i$ along the ray $\bfR \bfeta$ from the robot position $\bfp$ to the observed range $r$\NA{Should this be $r_{max}$?}. The set $\calR(\bfz ; \bfX, \bfeta)$ can be determined by a rasterization algorithm, such as Bresenham's line algorithm \cite{bresenham}.


\NA{Need to clean up from here on}

%Any mapping method is fundamentally a framework to integrate sensor data in order to provide a higher-level knowledge about the environment compared to raw sensor readings. For this aim, it is required to first specify the sensor model; which determines the association between the environment and any measurement made by the robot.

%Mapping is a probabilistic inference process that integrates sensory data to provide an incrementally refined distribution over possible environment realizations. For this aim, it is required to first specify the probabilistic sensor model~\eqref{eq:obs_model}, which determines the likelihood of measurements made by the robot.

%Given the robot pose $X_t$, the direction of a ray in the world frame can be obtained as $X_t \ubar{\eta}_b$, where $\ubar{\eta}_b$ is the homogeneous representation of $\eta_b$. Using a rasterization method, such as Bresenham's line algorithm \cite{bresenham}, we can find the indices of the map cells that intersect with a ray $\eta_b$.

\begin{proposition}
Let $z = (r,y)$ be a measurement made at time $t$ along a single ray $\eta_b$. The forward observation model $p(z \mid \bfm)$ is defined as:
% r -> r_max
\begin{equation}
    p(z \mid \bfm) = p(z) \prod_{i \in \calR_{t,b}(r)} \frac{p(m_i \mid z)}{p_0(m_i)},
\label{eq:forward_obs_model_semantic_decomp}
\end{equation}
%
where $\calR_{t,b}(r) \subseteq \calI$ is the set of indices of the map cells along the direction $X_t \ubar{\eta}_b$ that are observed by $z$.
\end{proposition}
%
Note that the set $\calR_{t,b}(r)$ is a function of the observation range $r$, meaning that only the cells located no farther than $r$ from the sensor are taken into account. The following definitions further specify the components of the observation model~\eqref{eq:forward_obs_model_semantic_decomp} for a measurement $z$ acquired at time $t$ along a single ray $\eta_b$.
%
\begin{definition}
The marginal observation model $p(z)$ is specified as the following:
%
\begin{equation}
    p(z) = \frac{p_0(m_{i_h} = y)}{\gamma(i_h)} \prod_{i \in \calR_{t,b}(r) \setminus \{i_h\}} p_0(m_i = 0),
\label{eq:marginal}
\end{equation}
%
where $i_h \in \calR_{t,b}(r)$ is the index of the cell hit by ray $\eta_b$ and $\gamma(i)$ denotes to the length of the intersection between direction $X_t \ubar{\eta}_b$ and map cell $m_i$. Fig.~\ref{??} illustrates the geometric interpretation of $\gamma(r)$. The ray continues to travel until it hits an obstacle or reaches its maximum range $r_{max}$. This results in:
%
\begin{equation}
    y \in \begin{cases}
    \calK \setminus \{0\} &\text{if}\; \calR_{t,b}(r) \subset \calR_{t,b}(r_{max}) \\
    \calK &\text{if}\; \calR_{t,b}(r) = \calR_{t,b}(r_{max})
    \end{cases}.
\end{equation}
%
\end{definition}
%
\begin{definition}
The inverse observation model is defined as a piece-wise constant function:
%
\begin{equation}
    p(m_{i} = k \mid z) =
    \begin{cases}
    \sigma^k(\bfl^+(y)) & \text{$z$ indicates class $y$} \\
    \sigma^k(\bfl^-) & \text{$z$ indicates free} \\
    \sigma^k(\bfl^0) & \text{otherwise}
    \end{cases},
\label{eq:semantic_inv_obs_model}
\end{equation}
%
where the parameters $\bfl^+(y)$, $\bfl^-$, and $\bfl^0$ represent the sensor noise specifications and $\sigma(\cdot)$ is the softmax function defined below.
\end{definition}
%
\begin{definition}
The softmax function $\sigma(\cdot): \bbR^{K+1} \rightarrow \bbR^{K+1}$ has the following properties:
%
\begin{equation}
\begin{split}
    \sigma(\bfl) &= [\sigma^0(\bfl), \sigma^1(\bfl), \ldots, \sigma^K(\bfl)]^T \\
    \sigma^k(\bfl) &= \frac{\exp{l_k}}{\sum_{k' \in \mathcal{K}} \exp{l_{k'}}} \\
    \log{\frac{\sigma^k(\bfl)}{\sigma^{k'}(\bfl)}} &= l_k - l_{k'}
\end{split}
\end{equation}
%
\end{definition}
%
In order to justify our selection for Eq.~\eqref{eq:forward_obs_model_semantic_decomp}, we start by employing the Bayes rule on the forward observation model:
%
\begin{equation}
    p(z \mid \bfm) = \frac{p(\bfm \mid z) p(z)}{p_0(\bfm)}.
\label{eq:forward_obs_model_semantic}
\end{equation}
%
We assume that a ray $z$ only depends on the subset of map cells $m_i$ where $i \in \calR_{t,b}(r)$. Moreover, without significant loss of accuracy, we assume that map cells are independent. This is illustrated in the graphical model shown in Fig.~\ref{}. Let $\calZ$ be a finite (possibly empty) set of observations. Based on this graphical model we have:
%
\begin{equation}
\begin{aligned}
    p(\bfm \mid \calZ) &= &&{\prod}_{i=1}^{N} p(m_i \mid \calZ) \\ &= &&{\prod}_{i \in \calR^\setC(\calZ)} p_0(m_i) {\prod}_{j \in \calR(\calZ)} p(m_j \mid \calZ)
\end{aligned}
\label{eq:map_ind}
\end{equation}
%
where $\calR(\calZ) \subseteq \calI$ is the set of indices of the map cells collectively observed by elements of $\calZ$ and $\calR^\setC(\calZ)$ denotes to the complement of $\calR(\calZ)$. Applying Eq.~\eqref{eq:map_ind} to the forward observation model~\eqref{eq:forward_obs_model_semantic} yields the structure presented in Eq.~\eqref{eq:forward_obs_model_semantic_decomp}.

Let $\bfl_i(z) = [0, l_{i,1}(z), \ldots, l_{i,K}(z)]^T$ be the vector of log ratios of the inverse observation model $p(m_i = k \mid z)$, i.e.:
%
\begin{equation}
    \log{\frac{p(m_i = k \mid z)}{p(m_i = 0 \mid z)}} = l_{i,k}(z) \;\;\; k \in \mathcal{K}.
\label{eq:log_inverse_obs_model}
\end{equation}
%
The inverse observation model for each class $k$ can then be recovered using a softmax function as $p(m_i = k \mid z) = \sigma^k(\bfl_i(z))$. Therefore, the inverse observation model can effectively be defined by imposing a structure on the log ratio vector $\bfl_i(z)$. This explains the formulation presented in Eq.~\eqref{eq:semantic_inv_obs_model} by assigning $\bfl_i(z)$ to one of $\bfl^+(y)$, $\bfl^-$, or $\bfl^0$ based on what $z$ indicates about $m_i$. Particularly, we define $\bfl^+(y)$ in a way that it accounts for both class prediction uncertainty and sensor noise as below:
%
\begin{equation}
\begin{split}
    l^+_k(y) = \phi^+_k &+ 
    \begin{cases}
    \psi_k & k = y \\
    0 & k \neq y
    \end{cases} \\
    \bfphi^+ = [0, \phi^+_1, \ldots, \phi^+_K]^T \;&\; \bfpsi = [0, \psi_1, \cdots, \psi_K]^T.
\end{split}
\end{equation}
%
If $z$ indicates that $m_i$ is occupied and belongs to the class $k$, the log ratio of class $k$ increases by $\phi^+_k + \psi_k$; however, we also increase the log ratio of other object classes by a smaller value $\phi^+_{k'}$ in order to account for the event that the sensor has incorrectly predicted the object class. The same formulation can be used if $z$ indicates that $m_i$ is free, hence:
%
\begin{equation}
    \bfl^- = \bfphi^- = [0, \phi^-_1, \ldots, \phi^-_K]^T.
\end{equation}
%
In this case, all elements of $\bfl^-$ should be non-positive in order to effectively increase the probability of $m_i$ being free. If $z$ does not carry any information about $m_i$, we simply consider the prior probabilities for the log ratio:
%
\begin{equation}
    l^0_k = \log{\frac{p_0(m_i = k)}{p_0(m_i = 0)}}.
\label{eq:log_prior}
\end{equation}
%
This completes the specification of the semantic observation model of Eq.~\eqref{eq:forward_obs_model_semantic_decomp}. Fig.~\ref{} shows each component of the observation model $p(z \mid \bfm)$ for a binary ($K = 1$) environment.






